Pairwise-Constrained Implicit Functions for 3D Human Heart Modelling

Accurate 3D models of the human heart require not only correct outer surfaces but also realistic inner structures, such as the ventricles, atria, and myocardial layers. Approaches relying on implicit surfaces, such as signed distance functions (SDFs), are primarily designed for single watertight surfaces, making them ill-suited for multi-layered anatomical structures. They often produce gaps or overlaps in shared boundaries. Unsigned distance functions (UDFs) can model non-watertight geometries but are harder to optimize, while voxel-based methods are limited in resolution and struggle to produce smooth, anatomically realistic surfaces. We introduce a pairwise-constrained SDF approach that models the heart as a set of interdependent SDFs, each representing a distinct anatomical component. By enforcing proper contact between adjacent SDFs, we ensure that they form anatomically correct shared walls, preserving the internal structure of the heart and preventing overlaps, or unwanted gaps. Our method significantly improves inner structure accuracy over single-SDF, UDF-based, voxel-based, and segmentation-based reconstructions. We further demonstrate its generalizability by applying it to a vertebrae dataset, preventing unwanted contact between structures.

==> bib/figmacro.tex <==
\newif\ifrgb
\rgbfalse

\newif\iffig
\figtrue

\newcommand{\figx}[2]
{
 \iffig
  \includegraphics[width=#1,keepaspectratio]{#2} 
 \else
   \parbox{#1}{#2} 
 \fi
}

\newcommand{\figy}[2]
{
 \iffig
  \includegraphics[height=#1,keepaspectratio]{#2}  
   \else
  \parbox{#1}{#2} 
 \fi
}

\newcommand{\figxy}[3]
{
 \iffig
  \includegraphics[width=#1,height=#2]{#3} 
 \else
   \parbox{#1}{#2}
  \fi
}

\newcommand{\figurecaption}[2]
{
\caption[]{\parbox[t]{#1}{#2}}
}

\newcommand{\fcaption}[1]
{
 \figurecaption{0.9\linewidth}{\small #1}
}

\newcommand{\figdir}[1]
{
\def\figurepath{#1}
}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}


==> figs/fail.tex <==
\begin{figure*}[]
    \begin{center}
    %\includegraphics[width=1\linewidth,height=5cm]{rebuttal/fail1.pdf} 
    %\makebox[0.48\linewidth]{(a) }
    \includegraphics[width=1\linewidth,height=5cm]{figs/fail2.pdf} 
    %\makebox[0.48\linewidth]{(b) }
    \makebox[0.32\linewidth]{(a) Ground-truth }
    \makebox[0.32\linewidth]{(b) Individual}
    \makebox[0.32\linewidth]{      (d) Jointly (Ours) }
    
    \end{center}
    \caption{\textbf{A failure case of our method.} Our method can resolve most of the topologically incorrect areas. However, there may remain small subsets of points that violate the constraints while being challenging to identify.
    } 
    \label{fig:fail}
    \end{figure*}
    

==> figs/heart_parts.tex <==
\begin{figure*}[]
    \begin{center}
    
    \includegraphics[width=\linewidth]{figs/supfigs/heartparts.pdf} 
    \makebox[0.45\linewidth]{(a) Side view }
    \makebox[0.45\linewidth]{(b) Top-down view}

    \end{center}
    \vspace{-3mm}
    \caption{\textbf{Different Human Heart Components.}  We show the reconstructed heart components from the baseline in the top row and our method in the middle row. The ground-truth is shown the bottom row. Green depicts proper contact while red means penetration.
    } 

    \label{fig:heart-parts}
    \end{figure*}
    

==> figs/heart_qual.tex <==
\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=0.46\linewidth]{figs/redraw_fig2.pdf}
    \includegraphics[width=0.46\linewidth]{figs/3b.pdf}
    \makebox[0.45\linewidth]{(a) Left-ventricle and its myocardium.}
    \makebox[0.45\linewidth]{(b) Right atrium and right ventricle.}% The bottom part is rotated }
    \end{center}
    %\vspace{-5mm}
    \caption{From left to right: the ground-truth 3D meshes, the reconstructed meshes using the baseline method deep-SDF, and the reconstructed 3D meshes using our method. The contact surfaces are colored green while the intersecting surfaces are colored red. %The contact and intersection ratios are shown next to the plots.
    \TODO{redraw}
    } 

    \label{fig:heart_qual}
    \end{figure*}

==> figs/mesh.tex <==
\begin{figure*}[]
    \begin{center}
    
    \includegraphics[width=\linewidth]{figs/meshOperation.pdf} 
    \makebox[0.24\linewidth]{(a) Ground-truth }
    \makebox[0.24\linewidth]{(b) DeepSDF}
    \makebox[0.24\linewidth]{(c) Mesh modification}
    \makebox[0.24\linewidth]{      (d) Ours }
    \end{center}
    \vspace{-3mm}
    \caption{\textbf{Comparison with explicit mesh modification.}  Starting from meshes obtained via DeepSDF, we select violated vertices and move them along their surface normal to resolve object-penetration. This approach yields rough surfaces with increased reconstruction errors. The numbers on the top-right corner indicates chamfer distances ($\times10e4$).
    } 
    \vspace{-5mm}
    \label{fig:mesh}
    \end{figure*}
    

==> figs/overview.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{figs/test.pdf} 
\makebox[0.20\linewidth]{(a) Initial State }
\makebox[0.3\linewidth]{(b) Point Sampling }
\makebox[0.3\linewidth]{(c) SDF Modification }
\makebox[0.15\linewidth]{(d) Output }
\end{center}
\caption{\textbf{Method overview.}  (a) We start with shapes defined by their respective SDFs~\cite{Park19c}  and parameterized by a latent vector. (b) We uniformly sample points around them. (c) We select a subset of topologically meaningful points such as ones residing close the object surfaces and use them to write loss functions. (d) We minimize these loss functions with respect to the latent vectors to enforce the constraints.}
\label{fig:overview}
\end{figure*}


==> figs/paralel.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[h!]
\begin{center}
%\includegraphics[width=0.7\linewidth]{figs/Overview_p1.pdf}
%\includegraphics[width=0.29\linewidth]{figs/Overview_p2.pdf}
\includegraphics[width=\linewidth]{figs/skin2.pdf} 
\makebox[0.3\linewidth]{(a)}
\makebox[0.3\linewidth]{(b)}
\makebox[0.3\linewidth]{(c)}
\end{center}
\vspace{-3mm}
\caption{\textbf{Reconstructing thin layers.} In each case, the image to the right is a magnified version of part of the image on the left.  (a) Fitting two layers separately. Note the yellow dot that denotes the  inner surface penetrating the outer one. (b) Fitting the layers jointly while imposing the parallel constraints. (c) Ground truth with voxels belonging to different layers painted in different colors. }
\label{fig:3dcontour}
\vspace{-5mm}
\end{figure*}

==> figs/refine.tex <==
\begin{figure*}[h]
    \begin{center}
    \includegraphics[width=0.22\linewidth, height=3cm]{figs/heart_refine/h300_L01.png} 
    \includegraphics[width=0.22\linewidth, height=3cm]{figs/heart_refine/h300_L00.png} 
    \includegraphics[width=0.22\linewidth, height=3cm]{figs/heart_refine/h200_L00.png} 
    \includegraphics[width=0.22\linewidth, height=3cm]{figs/heart_refine/h200_L01.png} 
    \makebox[0.22\linewidth]{nn-Unet}
    \makebox[0.22\linewidth]{Ours}
    \makebox[0.22\linewidth]{nn-Unet}
    \makebox[0.22\linewidth]{Ours}
    
    \end{center}
    \vspace{-3mm}
    \caption{\textbf{Heart Reconstruction from two Out-of-Distribution samples.} The nn-Unet result contains many mistakes, which our approach fixes. }
    \vspace{-5mm}
    \label{fig:refine}
    \end{figure*}
    

==> figs/spine/spine_sup.tex <==
\begin{figure*}[t]
    \begin{center}
    %\includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/spine00_L04.png}
    %\includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/spine00_L03.png}
   % \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/spine00_L01.png}
    %\includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/spine00_L02.png}
    %\includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/spine00_L00.png}
    %\includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/spine00_L07.png}
    %\includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/spine00_L05.png}
    %\includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/spine00_L06.png}

    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/800_L03.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/800_L02.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/800_L00.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/800_L01.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/500_L03.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/500_L02.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/500_L00.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/500_L01.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/300_L01.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/300_L00.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/300_L03.png}
    \includegraphics[width=0.24\linewidth, height=2cm]{figs/spine/300_L02.png}
    \makebox[0.24\linewidth]{(a) nn-Unet}
    \makebox[0.24\linewidth]{(b) Individual}
    \makebox[0.24\linewidth]{(c) Constrained (Ours)}
    \makebox[0.24\linewidth]{(d) Ground-Truth}
    
    \end{center}
    \vspace{-3mm}
    \caption{\textbf{3D Verterbea refinement via Implicit Functions.} (a) shows the segmentation results from nn-Unet. (b) depicts the resulting shapes when fitting implicit functions to each individual nn-Unet segmentation part, and (c) shows the results when fitting all parts simultaneously, with constraints enforced via our method. Areas in yellow indicate points in close proximity to other shapes, while areas in green highlight instances of touching, which should not occur.
    \vspace{-5mm}
    } 
    \label{fig:spine-sup}
    \end{figure*}
    

==> figs/teaser.tex <==
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=\linewidth]{figs/teaser.pdf}
    %\makebox[0.48\linewidth]{(a) 3D Annotations}
    %\makebox[0.48\linewidth]{(b) 2D}
    \end{center} 
    %\vspace{-4mm}
    \caption{
    \textbf{A 3D annotation of a human heart components. Right column shows a 2D slice of it. } Different components of the heart closely touch each other without intersecting, representing the constraint our method enforces.% This is challenging to model with implicit shape model \cite{Park2019deepSDFLC}.  
    }  %\vspace{-2pt}
    \label{fig:teaser} 
    \end{figure}

==> figs/teaser2.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\def \figlen{0.24\linewidth} 
\begin{figure}[t]
    \begin{center}
    \makebox[\figlen]{(a) GT in a 2D slice}
    \makebox[\figlen]{(b) 3D GT}
    \makebox[\figlen]{(c) DeepSDF}
    \makebox[\figlen]{(d) Ours}

    \includegraphics[clip,width=\linewidth]{figs/teaser/teaser4.pdf}
    \end{center} 
    \vspace{-4mm}
    \caption{
    \textbf{Topological Constraints in Composite Organs.}  (a) Ground-truth in a 2D MRI slice for the left ventricle and its myocardium at the top, and vertebrae L2 and L3 at the bottom. (b) Ground-truth in 3D.  In the top row, we show the same volume twice, once with only the left-ventricle and second time with only the myocardium for better visibility of the contact areas. 
    The contact ratio between the two is 27\% and that remains fairly constant across people. In the bottom row, there must be a minimum gap between L2 and L3. (c) The output surfaces when fitting DeepSDF~\cite{Park20a} to the nn-UNet~\cite{IsenseeEmail18} output and (d) when using our approach to fit the same  nn-UNet output. In (c,d), green denotes contact, red - intersection,  and yellow - proximity. For the myocardium, using DeepSDF yields intersections and the contact areas are random, whereas in our case there are no intersections and the contact area is properly shaped. For the vertebrae, we eliminate the contacts and areas of close proximity are properly modeled. }
    \vspace{-5mm}
    \label{fig:teaser} 
\end{figure}


==> secs/2_related_work_bak.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\section{Related Work}
%\TODO{check more recent work}
\paragraph{Image-Based Topological Interaction.}
Many 2D segmentation problems involve semantic classes with relative topology constraints between them, such as road connectivity over a background or cell nuclei that should be contained within the cytoplasm. For example,  a topology-aware loss that uses the response of selected filters from a pre-trained VGG19 network is introduced in \cite{Mosinska18}. These filters prefer elongated shapes and promote better connectivity. Similarly, a topology loss based on persistent diagrams is used in~\cite{hu2019topology}  to improve cell segmentation. Other methods rely on detecting and penalizing critical pixels for topology interaction between classes, such as \cite{Hu2021StructureAwareIS} and \cite{gupta2022learning}, using homotopy warping and convolutions respectively to find these pixels.
However, image and pixel based topology constraints do not lend themselves naturally to implicit multi-object 3D reconstruction. %To the best of our knowledge, our method is the first to define and enforce the contact ratio and minimum distances between components of 3D composite objects.

\paragraph{Multi-Object 3D Reconstruction.}
It is a fundamental task for scene understanding or generation~\cite{Irshad2022CenterSnapSM,Liu2021Voxelbased3D}. The presence of multiple objects poses a different set of challenges compared to single-object reconstruction where objects are usually treated as isolated geometries without considering the scene context, such as object locations and instance-to-instance interactions. For multi-object reconstruction, Mesh R-CNN~\cite{gkioxari2019meshrcnn} augments Mask R-CNN~\cite{he2017maksrcnn} with a mesh predictions branch that estimates a 3D mesh for each detected object in an image. Total3DUnderstanding~\cite{nie2020total} presents a framework that predicts room layout, 3D object bounding boxes, and meshes for all objects in an image based on the known 2D bounding boxes. However, these three methods first detect objects in the 2D image, and then independently produce their 3D shapes with single object reconstruction modules.
\cite{Liu2021Voxelbased3D} proposes a system to infer the pose, size, and location of 3D bounding boxes and the 3D shapes of multiple object instances in the scene, which is divided into a grid whose cells are occupied by objects.
\cite{irshad2022shapo} recovers objects shape, appearance, and poses using implicit representations, as has become increasingly frequent, \textit{e.g.}, \cite{irshad2022shapo,karunratanakul2020grasping,Ye2022WhatsIY,de2023drapenet}. For the most part, these works focus on reconstruction accuracy while our work focuses on the correctness of the topological constraints between components.

%\iffalse
\paragraph{3D Interactions.}
Some methods try to enforce consistency between objects in a scene when performing a 3D reconstruction, as in~\cite{Engelmann2020FromPT}  where a collision loss between reconstructed objects is minimized.  However, most such efforts 
focus on human-object interactions. In~\cite{karunratanakul2020grasping},  the grasp between the hand and an object is modeled in terms of implicit surfaces and the algorithm learns to generate new grasps using a VAE. The method of~\cite{Ye2022WhatsIY} jointly reconstructs  the hand-object interaction from an image and the object as an implicit surface. Contact2Grasp~\cite{li2023contact2grasp} learns to synthesize grasps by first predicting a contact map on the object surfaces. Other research directions include body-garment interaction, such as DrapeNet~\cite{de2023drapenet} with a physically based self-supervision, or human-scene interaction \cite{Hassan2020Populating3S}.
%\fi
%
All these works primarily focus on interactions between the articulated human body and objects, without incorporating any prior information on how they should interact. In contrast, our approach considers a specific topological and geometric constraint that needs to be hold between objects.%, such as a target contact ratio.

%Despite advances in deep learning-based 3D reconstruction, existing methods remain inadequate for this task. Voxel-based approaches, such as nn-UNet, are inherently limited by input voxel resolution, preventing them from modeling smooth, high-fidelity surfaces. Mesh-based methods can produce detailed geometries, but they often lack topological consistency, requiring manual corrections to fix misaligned or disconnected regions. More recently, implicit function representations, particularly signed distance functions (SDFs), have gained popularity due to their ability to model continuous, high-resolution surfaces. However, SDFs are primarily designed for single watertight surfaces, making them ill-suited for complex multi-layered structures like the heart. When applied to composite anatomical shapes, they fail to preserve shared boundaries, leading to gaps, unnatural overlaps, or disconnected components. Unsigned distance functions (UDFs), while capable of modeling non-watertight surfaces, suffer from unstable optimization, making them unreliable for medical applications. Several implicit function-based methods have been proposed for multi-component anatomical modeling, but they remain insufficient for heart reconstruction. Some recent works have explored implicit modeling of multi-component anatomical structures, but they remain insufficient for heart reconstruction. Implicit morphable models have been successfully applied to dental structures, where each component is treated independently, focusing on overall shape representation rather than ensuring accurate anatomical interfaces. More recent approaches, such as MODIF [arxiv:2312.10246], introduce multi-object implicit functions with inter-object constraints to prevent interpenetration and ensure spatial relationships between adjacent structures. However, these methods primarily focus on avoiding overlap rather than explicitly modeling shared surfaces with anatomical accuracy, making them unsuitable for the heart, where adjacent chambers must seamlessly form interconnected walls rather than merely avoiding collisions.

==> tabs/heart_reconstruction.tex <==

\begin{table*}[th]
    \centering
    \caption{{\bf Heart reconstruction.} We report the average surface penetration P.(\%) (lower is better), the average absolute difference from the ground-truth contact ratio $|\Delta\textrm{CT}|$ (lower is better), and Chamfer distance. Shapes generated using the baseline tend to intersect each other while having lower contact ratios than those obtained by optimizing all parts jointly and imposing the constraints. Shapes from nn-Unet exhibit correct topology but are extremely inaccurate for OOD samples.}
    %\vskip 0.1in
    \vspace{-0mm}
    \label{table:heart_quan}
    \begin{tabular}{cccccccc}
    %\toprule
    \multirow{2}{*}{Method}& \multicolumn{2}{c}{LV - MLV} & \multicolumn{2}{c}{LV-LA} &\multicolumn{2}{c}{MLV-RV} & All \\
    \cmidrule(lr){2-3}  
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-8}
     & P.(\%) & $|\Delta\textrm{CT}|$  (\%)  & P.(\%) & $|\Delta\textrm{CT}|$ (\%) & P.(\%) & $|\Delta\textrm{CT}|$ (\%)  & CD ($\times10^3$) \\
    \cmidrule(lr){1-1}  
    \cmidrule(lr){2-3}  
    \cmidrule(lr){4-5}  
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-8}
    &\multicolumn{7}{c}{In-distribution samples from public test set}\\
    \cmidrule(lr){1-8}  
    nn-Unet        & 0.0    & $0.1$  & 0.0   & $0.1$  & 0.0   & $0.1$& 0.3 \\       
    Individual       & 11.1 & $11.7$  & 1.7 & $2.7$ & 3.2 & $3.6$& 0.4 \\
    %deepSDF +M.M.  & 0.0 & 26.0   & 0.0 & 7.0 & 0.0 & 5.0& 15.6 \\   
    Joint (Ours)           & 0.0 & $0.1$   & 0.0 & $0.1$  & 0.0 &0.0 & \textbf{0.3} \\
    \midrule
    &\multicolumn{7}{c}{Out-of-distribution samples from private test set}\\
    \cmidrule(lr){1-8}  
    nn-Unet         & 0.0    & $0.8$  & 0.0   & $1.9$ & 0.0   & $0.3$& 46.8 \\       
    Individual      & 11.2 & $14.7$  & 1.7 & $2.7$ & 2.8 & $3.6$& 3.6 \\
    Joint (Ours)    & 0.2 & $4.4$   & 0.3 & $0.3$ & 0.4 &$1.0$ & \textbf{3.1} \\
    \midrule
    %\cmidrule(lr){1-8}  
    %GT (raw values)          & - & {27.0} & -  & {5.0}  &- & {4.7 }& - \\
    %\bottomrule
    \end{tabular}
    \vspace{-0mm}
\end{table*}

==> tabs/heart_reconstruction_raw.tex <==
\begin{table*}[th]
    \centering
    \caption{{\bf Heart reconstruction.} We report the average surface penetration (\%) (lower is better), contact ratio (\%) (closer to the ground truth is better), and chamfer distance (lower is better). Shapes generated from a vanilla deep-SDF model tends to intersect each other while having lower contact ratios.}
    %\vskip 0.1in
    %\vspace{-5mm}
    \label{table:heart_quan_raw}
    \begin{tabular}{lccccccc}
    %\toprule
    \multirow{2}{*}{Method}& \multicolumn{2}{c}{LV - MLV} & \multicolumn{2}{c}{LV-LA} &\multicolumn{2}{c}{MLV-RV} & All \\
    \cmidrule(lr){2-3}  
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-8}
     & Pen.(\%) & Cont.(\%)  & Pen.(\%) & Cont.(\%)& Pen.(\%) & Cont.(\%) & CD ($\times10^3$) \\
    \cmidrule(lr){1-1}  
    \cmidrule(lr){2-3}  
    \cmidrule(lr){4-5}  
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-8}
    &\multicolumn{7}{c}{In-distribution public test set}\\
    \cmidrule(lr){1-8}  
    nn-Unet        & -    & 26.9  & -   & 4.9 & -   & 4.8& 0.3 \\       
    deepSDF        & 11.1 & 15.3  & 1.7 & 2.3 & 3.2 & 1.1& 0.4 \\
    Ours           & 0.0 & 27.1   & 0.0 & 4.9 & 0.0 &4.7 & \textbf{0.3} \\
    \midrule
    &\multicolumn{7}{c}{Out-of-distribution private test set}\\
    \cmidrule(lr){1-8}  
    nn-Unet        & -    & 26.2  & -   & 6.9 & -   & 5.0& 46.8 \\   
    deepSDF        & 11.2 & 12.3  & 1.7 & 2.3 & 2.8 & 1.1& 3.6 \\
    Ours           & 0.2 & 22.6   & 0.3 & 4.7 & 0.4 &3.7 & \textbf{3.1} \\                   
    \cmidrule(lr){1-8}  
    GT             & - & 27.0 & -  & 5.0  &- &4.7 & - \\
    \bottomrule
    \end{tabular}
    \vspace{-0mm}
\end{table*}

==> tabs/spine_long.tex <==

\begin{table*}[th]
    \centering
    \caption{{\bf Spine reconstruction.} We report the average surface penetration (\%) (lower is better), contact ratio (\%) (closer to the ground truth is better), and chamfer distance (lower is better). Shapes generated from a vanilla deep-SDF model tends to intersect each other while having lower contact ratios.}
    %\vskip 0.1in
    %\vspace{-5mm}
    \label{table:heart_quan}
    \begin{tabular}{lccccccccc}
    %\toprule
    \multirow{2}{*}{Method}& \multicolumn{2}{c}{L1 - L2} & \multicolumn{2}{c}{L2 - L3} &\multicolumn{2}{c}{L3 - L4}&\multicolumn{2}{c}{L4 - L5} & All \\
    \cmidrule(lr){2-3}  
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-9}
    \cmidrule(lr){10-10}
     & px$^2$ & N  & px$^2$ & N & px$^2$ & N &px$^2$ & N  & CD ($\times10^3$) \\
    \cmidrule(lr){1-1}  
    \cmidrule(lr){2-3}  
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-9}
    \cmidrule(lr){10-10}
    nn-Unet        & 261.39 & 123.17 & 527.23  & 237.34 & 644.58 & 294.32 & 761.06 & 358.93 & 0.35   \\       
    deep-SDF        & 315.84 & 154.17 & 309.77  & 166.06& 416.43 & 227.65 & 503.31 & 279.43 & 0.44   \\                                 
    Ours           & \textbf{0.04} & \textbf{0.76} & \textbf{0.45}  & \textbf{2.32}& \textbf{0.53 }& \textbf{2.89 }& \textbf{1.19 }& \textbf{3.89 }& \textbf{0.30}   \\                   
    \bottomrule
    \end{tabular}
    \vspace{-0mm}
\end{table*}

==> tabs/wall.tex <==
\begin{table}[]
\centering
\caption{{\bf Reconstructing outer-inner objects.} The inner object surface is expected to be in a distance of 2-4 pixels from the outer object surface.}
\vskip 0.1in
\label{table:wall}
\centering
\begin{tabular}{ccccccc} % <-- Removed two 'c' specifiers
    \toprule
    \multirow{2}{*}{Component} & \multicolumn{2}{c}{Violation (N.o. Vertices)}&\multirow{2}{*}{ Total Vertices}  \\
    \cmidrule(lr){2-3}
    & deepSDF & Ours \\
    \midrule
    \pz & 4638.94 & 145.80 & 132104.5\\
    \po & 1170.26 & 0.00 & 43932.0\\
    \ptw & 2020.36 & 0.00 & 60126.6\\
    \pth & 1267.76 & 55.66 & 36288.4 \\
    Right-Ventricle & 1547.81 & 16.59 & 67140.2\\
    \bottomrule
\end{tabular}
\end{table}

